Error Correction in Learning using SVMs

This paper is concerned with learning binary classifiers under adversarial label-noise. We introduce the problem of error-correction in learning where the goal is to recover the original clean data from a label-manipulated version of it, given (i) no constraints on the adversary other than an upper-bound on the number of errors, and (ii) some regularity properties for the original data. We present a simple and practical error-correction algorithm called SubSVMs that learns individual SVMs on several small-size (log-size), class-balanced, random subsets of the data and then reclassifies the training points using a majority vote. Our analysis reveals the need for the two main ingredients of SubSVMs, namely class-balanced sampling and subsampled bagging. Experimental results on synthetic as well as benchmark UCI data demonstrate the effectiveness of our approach. In addition to noise-tolerance, log-size subsampled bagging also yields significant run-time benefits over standard SVMs.

==> Proof.tex <==
\section{Proof for optimality of class-balanced sampling ($p=0.5$)}
\label{sec:proof}
Consider a two-class classification problem where the two classes are represented by $A$ and $B$. Without loss of generality, let $A$ be the minority class containing $0<\beta\leq0.5$  fraction of the points. Let $\widehat{A}$ and $\widehat{B}$ represent the two classes after one or both the classes are corrupted with adversarial noise. Let $\rho\beta,~0\leq\rho<1$ represent the upper limit on the fraction of corrupted points. Therefore, the total number of corrupted points can be written as $n_c = \rho\beta\l$. Further, let $alpha$ be the fraction of the corrupted points that were originally in class $B$ but were assigned to class $A$. Therefore, the fraction of the new classes can be given by
\begin{align}
|\widehat{A}| &= \beta + \alpha\rho\beta - (1-\alpha)\rho\beta\\
|\widehat{B}| &= 1 - \beta - \alpha\rho\beta + (1-\alpha)\rho\beta
\end{align}
Moreover, the fraction of good (clean) and bad (mislabeled) points in both the classes are
\begin{align}
|\widehat{A}_g| &= \beta - (1-\alpha)\rho\beta\\
|\widehat{A}_b| &= \alpha\rho\beta\\
|\widehat{B}_g| &= 1 - \beta - \alpha\rho\beta\\
|\widehat{B}_b| &= (1-\alpha)\rho\beta
\end{align}
Therefore, the conditional probability of picking a good or a bad point for both the classes are given by
\begin{align}
P(a_g|\widehat{A}) &= \frac{|\widehat{A}_g|}{|\widehat{A}|} = \frac{1 - (1-\alpha)\rho}{1 + \alpha\rho - (1-\alpha)\rho}\\
P(a_b|\widehat{A}) &= \frac{|\widehat{A}_b|}{|\widehat{A}|} = \frac{\alpha\rho}{1 + \alpha\rho - (1-\alpha)\rho}\\
P(b_g|\widehat{B}) &= \frac{|\widehat{B}_g|}{|\widehat{B}|} = \frac{1 - \beta - \alpha\rho\beta}{1 - \beta - \alpha\rho\beta + (1-\alpha)\rho\beta}\\
P(b_b|\widehat{B}) &= \frac{|\widehat{B}_b|}{|\widehat{B}|} = \frac{(1-\alpha)\rho\beta}{1 - \beta - \alpha\rho\beta + (1-\alpha)\rho\beta}
\end{align}
Assuming that the probability with which points from classes $\widehat{A}$ and $\widehat{B}$ are picked is given by $P(\widehat{A}) = p$ and $P(\widehat{B}) = 1-p$ respectively, the probability of picking up a good or a bad point for both the classes are respectively given by
$P(a_g) = P(a_g|\widehat{A})p$, $P(a_b) = P(a_b|\widehat{A})p$, $P(b_g) = P(b_g|\widehat{B})(1-p)$ and $P(b_b) = P(b_b|\widehat{B})(1-p)$.

The probability $\eta$ of not picking $r/2$ clean points from either class is upper bounded by
\begin{align}
\label{eqn:etaBinomial1}
\nonumber \eta \leq & \sum_{k=0}^{r/2-1} {s \choose k} \left(P(a_g)\right)^k \left(1 - P(a_g)\right)^{s-k} \\
+ & \sum_{k=0}^{r/2-1} {s \choose k} \left(P(b_g)\right)^k \left(1 - P(b_g)\right)^{s-k}.
\end{align}
For worst case analysis, we need to maximize $\eta$ and therefore, minimize both $P(a_g)$ and $P(b_g)$, which in turn requires minimizing $P(a_g|\widehat{A})$ and $P(b_g|\widehat{B})$ w.r.t. both $\alpha$ and $\beta$. Differentiating $P(a_g|\widehat{A})$ w.r.t $\alpha$
\begin{equation}
\frac{dP(a_g|\widehat{A})}{d\alpha} = \frac{\rho(-1 + \rho)}{(1 - \rho + 2\alpha\rho)^2} \leq 0.
\end{equation}
Therefore, 
\begin{equation}
\arg\min_\alpha P(a_g) = 1.
\end{equation}
Similarly, differentiating $P(b_g|\widehat{B})$ w.r.t. $\alpha$
\begin{equation}
\frac{dP(b_g|\widehat{B})}{d\alpha} = \frac{\rho\beta(1 - \beta(1+\rho))}{(1 - \beta + \rho\beta - 2\alpha\rho\beta)^2} \geq 0
\end{equation}
Therefore, 
\begin{equation}
\arg\min_\alpha P(b_g) = 0.
\end{equation}
Also,
\begin{equation}
\frac{dP(b_g|\widehat{B})}{d\alpha} = \frac{-\rho(1 - \alpha)}{(1 - \beta + \rho\beta - 2\alpha\rho\beta)^2} \leq 0
\end{equation}
implying that
\begin{equation}
\arg\min_\beta P(b_g) = \frac{1}{2} ~.
\end{equation}
Substituting $\alpha = 1$ in $P(a_g)$ and $\alpha = 0, \beta = 1/2$ in $P(b_g)$, we get
\begin{equation}
\min P(a_g) = \frac{p}{1+\rho} ~~~~\text{and}~~~~~ \min P(b_g) = \frac{1-p}{1+\rho}.
\end{equation}
Therefore, the worst case bound for (\ref{eqn:etaBinomial1}) can be written as
\begin{align}
\label{eqn:etaBinomial2}
\nonumber \eta \leq & \sum_{k=0}^{r/2-1} {s \choose k} \left(\frac{p}{1+\rho}\right)^k \left(1 - \frac{p}{1+\rho}\right)^{s-k} \\
+ & \sum_{k=0}^{r/2-1} {s \choose k} \left(\frac{1-p}{1+\rho}\right)^k \left(1 - \frac{1-p}{1+\rho}\right)^{s-k}.
\end{align}

Applying Hoeffding bound \cite{hoeffding63} individually on each of the two terms
\begin{align}
\label{eqn:etaHoeffding1}
\nonumber \eta \leq & \frac{1}{2} \exp{\left(-\frac{2}{s}\left(\frac{sp}{1-\rho} - \frac{r}{2} + 1\right)^2\right)} \\
+ & \frac{1}{2} \exp{\left(-\frac{2}{s}\left(\frac{s(1-p)}{1+\rho} - \frac{r}{2} + 1\right)^2\right)}
\end{align}
as long as $\frac{sp}{1+\rho} > \frac{r}{2} - 1$ and $\frac{s(1-p)}{1+\rho} > \frac{r}{2} - 1$. The RHS of \ref{eqn:etaHoeffding1} can be rewritten as 
\begin{align}
\label{eqn:etaHoeffding2}
\nonumber f = & \frac{1}{2}\exp\left(-\frac{1}{2}\left(\frac{p - \frac{(r-2)(1+\rho)}{2s}}{\left(\frac{1+\rho}{2\sqrt{s}}\right)}\right)^2\right) \\ 
+ & \frac{1}{2}\exp\left(-\frac{1}{2}\left(\frac{(1-p) - \frac{(r-2)(1+\rho)}{2s}}{\left(\frac{1+\rho}{2\sqrt{s}}\right)}\right)^2\right)
\end{align}
which is simply the sum of two Gaussian with means $\mu_1 = \frac{(r-2)(1+\rho)}{2s}$ and $\mu_2 = 1-\frac{(r-2)(1+\rho)}{2s}$ and equal variance $\sigma = \frac{1+\rho}{2\sqrt{s}}$. Differentiating the above expression w.r.t. $p$
\begin{align}
\label{eqn:df}
\nonumber \frac{df}{dp} = - & \frac{2\left(\frac{sp}{1 + \rho} - \frac{r}{2} + 1\right)}{\exp\left(\frac{2}{s}\left(\frac{sp}{1 + \rho} - \frac{r}{2} + 1\right)^2\right)(1 + \rho)} \\
+ & \frac{2\left(\frac{s(1 - p)}{1 + \rho} -\frac{r}{2} + 1\right)}{\exp\left(\frac{2}{s}\left(\frac{s(1 - p)}{1 + \rho} - \frac{r}{2} + 1\right)^2\right)(1 + \rho)}.
\end{align}
It can be clearly seen that $p=0.5$ is a solution of (\ref{eqn:df}). Also, the sum of two Gaussians can be either unimodal ($p=0.5$ is global maximum) or bimodal ($p=0.5$ is a minimum) \cite{behboodian70}. The second order derivative of $f$ w.r.t. $p$ can be written as
\begin{align}
\nonumber \frac{d^2f}{dp} = & \frac{8\left(\frac{sp}{1 + \rho} - \frac{r}{2} + 1\right)^2 - 2s}{\exp\left(\frac{2}{s}\left(\frac{sp}{1 + \rho} - \frac{r}{2} + 1\right)^2\right)(1 + \rho)^2} \\
+ & \frac{8\left(\frac{s(1 - p)}{1 + \rho} - \frac{r}{2} + 1\right)^2 - 2s}{\exp\left(\frac{2}{s}\left(\frac{s(1 - p)}{1 + \rho} - \frac{r}{2} + 1\right)^2\right)(1 + \rho)^2}.
\end{align}
Therefore, enforcing a minimum at $p=0.5$, we get the condition that
\begin{align}
\nonumber \frac{d^2f}{dp}\Big |_{p=0.5} = & \frac{32\left(\frac{s}{2(1 + \rho)} - \frac{r}{2} + 1\right)^2}{\exp\left(\frac{2}{s}\left(\frac{s}{2(1 + \rho)} - \frac{r}{2} + 1\right)^2\right)(1 + \rho)^2} \\
- & \frac{8s}{\exp\left(\frac{2}{s}\left(\frac{s}{2(1 + \rho)} - \frac{r}{2} + 1\right)^2\right)(1 + \rho)^2} \geq 0.
\end{align}
This directly implies that
\begin{equation}
s \geq (\rho + 1)\left(r -2 + \frac{1}{2}(\rho + 1)\left(1 + \left(\frac{4r + \rho - 7}{\rho + 1}\right)^{1/2}\right)\right)
\label{eqn:s-final}
\end{equation}
which, as expected, is a stronger condition than the one required for imposing the Hoeffding bound at $p = 0.5$, i.e., $s > (1+\rho)(r - 2)$. Furthermore, to enforce $p=0.5$ to be the \textit{global} minimum, we impose the condition that the value of $f$ at $p=0.5$ is strictly less than that at any of the two extreme points of $f$ (i.e., at $p = \frac{1}{s}(1+\rho)(r/2-1)$ and $p = 1 - \frac{1}{s}(1+\rho)(r/2-1)$). This gives us an even stronger condition
\begin{dmath}
s \geq (\rho + 1)\left(r -2 + (\rho + 1)\left(\log2 + \left(\frac{\log2(\log2 + 2r + \rho\log2 - 4)}{\rho + 1}\right)^{1/2}\right)\right).
\end{dmath}
This is the sufficient condition to guarantee that the worst case probability of selecting less than $r/2$ clean points per class is minimum at $p=0.5$, i.e., when \textit{class-balanced} sampling is performed over the data.

%
%
%\newpage
%\begin{eqnarray}
%(\rho + 1)\left(r -2 + \frac{1}{2}(\rho + 1)\left(1 + \left(\frac{4r + \rho - 7}{\rho + 1}\right)^{1/2}\right)\right)\\
%(\rho + 1)\left(r -2 + \frac{1}{2}(\rho + 1) + \frac{1}{2}(\rho + 1)\left(\frac{4r + \rho - 7}{\rho + 1}\right)^{1/2}\right)
%\end{eqnarray}
%
%\begin{eqnarray}
%(\rho + 1)\left(\log{2} + r + \rho\left(\frac{\log{2}(\log{2} + 2r + \log{2}\rho - 4)}{(\rho + 1)}\right)^{1/2} + \rho\log{2} + \left(\frac{\log{2}(\log{2} + 2r + \log{2}\rho - 4)}{(\rho + 1)}\right)^{1/2} - 2\right)\\
%(\rho + 1)\left(\log{2} + r + \rho\left(\frac{\log{2}(\log{2} + 2r + \log{2}\rho - 4)}{(\rho + 1)}\right)^{1/2} + \rho\log{2} - \left(\frac{\log{2}(\log{2} + 2r + \log{2}\rho - 4)}{(\rho + 1)}\right)^{1/2} - 2\right)\\
%\end{eqnarray}
%
%\begin{eqnarray}
%\nonumber
%1 + \exp\left(-\frac{2}{s}\left(\frac{s}{1+\rho} - r + 2\right)^2\right) ~~~~>~~~~
%2\exp\left(-\frac{1}{2s}\left(\frac{s}{1+\rho} - r + 2\right)^2\right)\\
%\end{eqnarray}
%
%\begin{align}
%\nonumber
%f_1 &= \exp\left(-\frac{2}{s}\left(\frac{sp}{1+\rho} - \frac{r}{2} + 1\right)^2\right)\\
%\nonumber
%    &= \exp\left(-\frac{1}{2}\left(\frac{2\sqrt{s}p}{1+\rho} - \frac{r}{\sqrt{s}} + \frac{2}{\sqrt{s}}\right)^2\right)\\
%\nonumber
%    &= \exp\left(-\frac{1}{2}\left(\frac{p}{\left(\frac{1+\rho}{2\sqrt{s}}\right)} - \left(\frac{r-2}{\sqrt{s}}\right)\right)^2\right)\\
%\nonumber    
%    &= \exp\left(-\frac{1}{2}\left(\frac{p - \left(\frac{r-2}{\sqrt{s}}\right)\left(\frac{1+\rho}{2\sqrt{s}}\right)}{\left(\frac{1+\rho}{2\sqrt{s}}\right)}\right)^2\right)\\
%\nonumber    
%    &= \exp\left(-\frac{1}{2}\left(\frac{p - \frac{(r-2)(1+\rho)}{2s}}{\left(\frac{1+\rho}{2\sqrt{s}}\right)}\right)^2\right)\\
%\nonumber    
%\end{align}
%
%Isn't this just a Gaussian with $\mu = \frac{(r-2)(1+\rho)}{2s}$ and $\sigma = \frac{1+\rho}{2\sqrt{s}}$ (although $p$ just varies between $[0,1]$)? Similarly, $f_2$ will be a Gaussian with $\mu = 1-\frac{(r-2)(1+\rho)}{2s}$ and $\sigma = \frac{1+\rho}{2\sqrt{s}}$.
%
%
%
%\newpage
%\begin{equation}
%\nonumber
%\frac{df}{dp} = - \frac{4\left(\frac{sp}{1 + \rho} - \frac{r}{2} + 1\right)}{\exp\left(\frac{2}{s}\left(\frac{sp}{1 + \rho} - \frac{r}{2} + 1\right)^2\right)(1 + \rho)} + \frac{4\left(\frac{s(1 - p)}{1 + \rho} -\frac{r}{2} + 1\right)}{\exp\left(\frac{2}{s}\left(\frac{s(1 - p)}{1 + \rho} - \frac{r}{2} + 1\right)^2\right)(1 + \rho)}
%\end{equation}
%
%\begin{equation}
%\nonumber
%\frac{d^2f}{dp} = \frac{16\left(\frac{sp}{1 + \rho} - \frac{r}{2} + 1\right)^2 - 4s}{\exp\left(\frac{2}{s}\left(\frac{sp}{1 + \rho} - \frac{r}{2} + 1\right)^2\right)(1 + \rho)^2} + \frac{16\left(\frac{s(1 - p)}{1 + \rho} - \frac{r}{2} + 1\right)^2 - 4s}{\exp\left(\frac{2}{s}\left(\frac{s(1 - p)}{1 + \rho} - \frac{r}{2} + 1\right)^2\right)(1 + \rho)^2}
%\end{equation}
%
%\begin{equation}
%\nonumber
%\frac{d^2f}{dp}\Big |_{p=0.5} = \frac{32\left(\frac{s}{2(1 + \rho)} - \frac{r}{2} + 1\right)^2}{\exp\left(\frac{2}{s}\left(\frac{s}{2(1 + \rho)} - \frac{r}{2} + 1\right)^2\right)(1 + \rho)^2} - \frac{8s}{\exp\left(\frac{2}{s}\left(\frac{s}{2(1 + \rho)} - \frac{r}{2} + 1\right)^2\right)(1 + \rho)^2}
%\end{equation}


==> related.tex <==
\section{Related Work}

\subsection{Related adversarial and noise models}
\label{sec:related-adversarial-models}

Learning in the presence of an adversary has been considered before in machine learning. For
example, \cite{DDMSV04} address the problem of coping with an active adversary who tries to defeat
a classifier (previously trained to give good performance) by carefully constructing new points on
which the classifier makes mistakes (Constructing emails that trick a spam filter is a typical
example). Spam-classification is viewed as a game between classifier and adversary, and algorithms are presented that produce
optimal classifiers against optimal adversarial strategies. Similarly, \cite{LM05a} introduce the
notion of Adversarial Classifier Reverse Engineering, where the adversary's goal is to identify high-quality points
that can slip through the classifier (or spam filter). The adversary must learn sufficient information to
mount such attacks by issuing only a reasonable (polynomial) number of queries to the classifier.
%These adversarial scenarios correspond to what can be referred to as {\em exploratory} attacks
%(\cite{BNSJT06}) and are different from our error-correction setting (which is basically a {\em
%causative} attack scenario).

Learning from data with adversarial (or worst-case) errors has been studied mainly in computational learning 
theory literature (see, e.g., \cite{KSS94,hastad97,FGKP06,GR06}). 
\cite{KSS94} show that under an `agnostic' PAC learning model (a generalization of the classical PAC learning model
based on weakening of target function assumptions) learning even simple concepts can be NP-hard. 
Similarly, \cite{hastad97} shows that learning parities in the presence of adversarial noise, under arbitrary distributions, is
intractable. There are also negative results concerning the hardness of learning halfspaces in the
presence of worst-case noise (\cite{GR06}).

Several noise models have been proposed that extend the noise-free setting in
the PAC model. For example, \cite{valiant85} and \cite{BGMST98} develop algorithms with theoretical
guarantees of learning from data with random {\em iid} noise. Many others 
evaluate performance through extensive empirical studies on randomly perturbed data sets
(see, e.g., \cite{AAP05,KK05,KW07}). However, as discussed earlier, such random noise models
are not suitable in an adversarial setting. A more compelling noise model was reported by
\cite{KL93} for learning in the presence of what they call as {\em malicious errors}.
Here, a random oracle chooses which
points in the data set to corrupt, but the adversary decides the actual corruption.
An even more powerful adversary, referred to as {\em nasty noise} was defined by \cite{BEK99}
where the adversary chooses both which points to corrupt and how to corrupt them,
the only restriction being that the number of corrupted points is a
binomial random variable. All these noise models lead to predominantly negative results - 
although some positive results exist for specific and simple learning algorithms under very
specialized settings. 

Recently, \cite{DS09} considered the problem of learning SVMs in a multi-teacher setting, where some teachers may be malicious. Each teacher is given a random set of examples from the underlying data distribution (that admits easy classification by SVM) and a small subset of teachers can be malicious (and can label their examples arbitrarily). They further assume that the malicious teachers do not know the identity of the good teachers' examples. The error-correction problem in learning also involves estimating classifiers from training data that may have been manipulated by an adversary and we also assume that in the absence of an adversary, the data distribution admits of effective classification using a standard SVM. However, unlike in \cite{DS09}, there is no explicit notion of multiple teachers and no assumption that the adversary has access to a random set of examples. Instead, we introduced the notion of adversarial intensity to model a wide variety of correlated errors (which includes, but is not limited to, worst-case errors). We presented an algorithm which can recover from nearly a constant fraction of correlated errors, provided the adversarial intensity is less than half.

%Learning from adversarial data has been studied in complexity theory for many years \cite{haussler92,KSS94}.
%Hardness of learning halfspaces in the presence of noise: (\cite{GR06}).
%New results for learning noisy parities and halfspaces: (\cite{FGKP06}).

%Learning with noise. Extension to regression: (\cite{teytaud01})
%Noise-tolerant variants of the perceptron algorithm (\cite{KW07}).

%Adversarial classification (in a game theoretic setting): (\cite{DDMSV04}).

%Adversarial learning where adversary can issue membership queries and has access to an adversarial
%cost function: (\cite{LM05a}).

%Pruning training sets for learning object categories (\cite{AAP05}).
%Boosting approach to removing class label noise (\cite{KK05}).

\subsection{Existing results on bagging}
\label{sec:existing-results-on-bagging}

Bagging (acronym for ``bootstrap aggregating'') was originally introduced by \cite{breiman96}
for improving accuracy of `unstable' predictors. For binary
classification\footnote{In general, bagging is relevant for both categorical as well as
numerical predictors. Here we review only bagging as applied to binary classifiers.}, the training data is
a set of (say $\ell$) input-output pairings, $\DB=\{(x_i,y_i)\::\:i=1,\ldots,\ell)\}, y\in\{-1,+1\}$.
%drawn {\em iid} according to some unknown data distribution $\scrD$,
Let $\Psi_\DB(\cdot)$ denote a classifier estimated from $\DB$.
Bagging constructs several replicate data sets (referred to as bootstrap samples) -- 
each consisting of $\ell$ input-output pairs drawn at random, with replacement, from
$\DB$. A predictor, $\Psi_{\DB^b}(\cdot)$, is estimated from each bootstrap sample, $\DB^b$,
and the final bagged decision for a point is given by a majority vote over all the bootstrapped predictors.
Several studies have investigated the question(s) of why (and under what conditions) bagging works (see, e.g.,
\cite{breiman96b}, \cite{BY02}, \cite{EEP05}). In general, these studies formalize 
different notions of stability for predictors and show that bagging
reduces the variance of unstable predictors. Other explanations for bagging (not involving a bias-variance
analysis) have also been reported. For example, \cite{SFBL98} relate the generalization error of voting methods to the margin distribution of training
examples. Based on analysis of U-statistics, \cite{BS00} qualify the effects of bagging on
variance, squared bias and mean squared error. On the other hand, instead of studying such global
effects of bagging on the base predictor, \cite{grandvalet04} argues that bagging
systematically equalizes the influence of training examples in the estimation process.

Many of these works also report results on common variants of bagging. For example, \cite{BY02} theoretically motivate subsampled bagging as being computationally more efficient, while achieving nearly the same accuracy as traditional bagging. Similarly, the equalization effect of training examples supports resampling strategies such as half-sampling which should be qualitatively identical to bootstrap sampling while being computationally less demanding (see \cite{grandvalet04}). Experimental bias-variance analysis of random aggregation and bagging of SVMs demonstrates that working with small samples achieves greater reduction in the variance component of error than standard bagging (see \cite{valentini04}). In another related work, \cite{BF99} presents an experimental study of various methods for identifying mislabelled data. The general idea is to split the data into $k$-folds for cross-validation, train an ensemble of classifiers on the training sets and then employ majority vote or consensus filters to determine the mislabelled instances. However, no theoretical results or performance guarantees are reported. All these studies, including the ones we discussed earlier, such as the analyses of regular bagging, assume that training examples are {\em iid} realizations from a fixed probability distribution -- an assumption that is not viable in our error-correction context. Also, these works do not consider the case of learning from data containing (potentially malicious) correlated errors (and typically consider only random independent label flips as the error model). By contrast, in this paper, we showed how class-balanced subsampled bagging of SVMs can be useful for error-correction in learning binary classifiers, where the errors may be maliciously introduced by an adversary (making it unreasonable to make any independence assumptions in the corruption process).



